HorNets: Learning from Discrete and Continuous Signals with Routing Neural Networks

Construction of neural network architectures suitable for learning from both continuous and discrete tabular data is a challenging research endeavor. Contemporary high-dimensional tabular data sets are often characterized by a relatively small instance count, requiring data-efficient learning. We propose HorNets (Horn Networks), a neural network architecture with state-of-the-art performance on synthetic and real-life data sets from scarce-data tabular domains. HorNets are based on a clipped polynomial-like activation function, extended by a custom discrete-continuous routing mechanism that decides which part of the neural network to optimize based on the input's cardinality. By explicitly modeling parts of the feature combination space or combining whole space in a linear attention-like manner, HorNets dynamically decide which mode of operation is the most suitable for a given piece of data with no explicit supervision. This architecture is one of the few approaches that reliably retrieves logical clauses (including noisy XNOR) and achieves state-of-the-art classification performance on 14 real-life biomedical high-dimensional data sets. HorNets are made freely available under a permissive license alongside a synthetic generator of categorical benchmarks.

==> generator.tex <==
Next, we describe our generator. Consider a set of input variables, denoted by $V$, and the set of binary operators $\mathcal{OP}$. For each combination of a variable $v \in V$ and an operator $o \in \mathcal{OP}$, we generate $N$ instances. Each instance, denoted $x_i$, for $i = 1, 2, \ldots, N$, is independently drawn from a Bernoulli distribution, specifically $x_i \sim \text{Bernoulli}(0.5)$, ensuring each bit $x_{i,j}$ (where $j = 1, 2, \ldots, |V|)$ is equally likely to be 0 or 1. These instances are then split into training and testing datasets, with a split ratio $\rho$ defined as $\rho_{\text{train}} = 0.7$ and $\rho_{\text{test}} = 0.3$, respectively. Thus, the number of training instances $N_{\text{train}}$ is computed as $\lceil \rho_{\text{train}} \cdot N \rceil$, and the number of testing instances $N_{\text{test}}$ is $\lfloor \rho_{\text{test}} \cdot N \rfloor$. The output dataset $D(v, o)$ comprises tuples $(x_i, o(x_i))$, where each $x_i$ is a vector in $\{0,1\}^{|V|}$ and $o(x_i)$ is the result of applying the operator $o$ to $x_i$. 

